Touchdown: Natural Language Navigation and Spatial Reasoning in Visual Street Environments

We study the problem of jointly reasoning about language and vision through a navigation and spatial reasoning task. We introduce the Touchdown task and dataset, where an agent must first follow navigation instructions in a real-life visual urban environment, and then identify a location described in natural language to find a hidden object at the goal position. The data contains 9,326 examples of English instructions and spatial descriptions paired with demonstrations. Empirical analysis shows the data presents an open challenge to existing methods, and qualitative linguistic analysis shows that the data displays richer use of spatial reasoning compared to related resources.

==> content/6-methods.tex <==
\section{Methods}
\label{sec:methods}

\subsection{Referring Expression Interpretation}



\ya{basic MLP}

\ya{text2conv}

\ya{lingunet?}


\subsection{Navigation Task} \dm{We evaluate our agent on the task of being able to follow the instruction to navigate in the map. We evaluate the agent using shortest-path demonstration (SD) from the final position of the agent after execution to the goal state.} 

\dm{Explain the Chaplot and Misra model}

\dm{Explain the decoupled attention model}

\subsection{Complete Task}

\ya{need to think if we can do anything here -- if navigation is getting something right, maybe can just pipeline}

==> content/7-exp.tex <==
\section{Experimental Setup}
\label{sec:expsetup}

\paragraph{Baselines} For the navigation task, we compare the models discussed in Section~\ref{sec:methods} against the following baselines: (a) STOP: Agent stops immediately; (b) RANDOM: Agent samples a non-stop action uniformly randomly from the action space and (c) FORWARD: Agent always takes the forward action. \dm{what else can we add}

\paragraph{Evaluation Metric} \dm{Howard add stuff here for other problem} For the navigation task, we evaluate the agent using the length of the shortest path from the final state of the agent to the goal state. We term this evaluation metric as ${\tt StopDist}$.

\paragraph{Reward Function} For the navigation task, the agent receives a reward $R(s, a, s')$ when moving from state $s$ to state $s'$ on taking action $a$. The reward $R(s, a, s')$ is the sum of a problem reward $R_p(s, a, s')$ defining the essence of the problem setup and a shaping reward term $F(s, a, s')$ intended to help the learning~\cite{Ng:99rewardshaping, Misra:17instructions}.  The problem reward $R_p(s, a, s')$ is given as follows:

\begin{equation}
    R_p(s, a, s') = \begin{cases}
      1, & \text{$a=STOP$ and $s'$ is the goal}\\
      -1, & \text{$a=STOP$ and $s'$ is not the goal}\\
      -\delta, & \text{otherwise} \\
    \end{cases}
\end{equation}

the shaped reward is given by $F(s, a, s') = \phi(s') - \phi(s)$ where the potential function $\phi(s)$ is the length of the shortest path from the state $s$ to the goal state. The shaping term incentivizes the agent if it moves closer to the goal state.

\paragraph{Hyperparameters} For the navigation task, we set the learning rate to 0.0025 and set the entropy coefficient to 0.1 for all reinforcement learning or contextual bandit settings.  \dm{image features etc.}



==> content/8-results.tex <==
\section{Results}
\label{sec:results}

\paragraph{Referring Expression Tasks} \dm{Explain the result}

\begin{table}[t]
\begin{center}\footnotesize
\begin{tabular}{ |c||c|c| }
 \hline
 Model & Mean Distance (pixel) & Accuracy (\%) \\
 \hline
 \imagetextconcat & $114.59$ & $17.19$\\ 
 \hline
 \imagetextconcatconv & $114.37$ & $17.60$ \\ 
 \hline
 \texttoconv & $97.69$ & $28.78$ \\ 
 \hline
 \lingunet & $91.46$ & $32.29$ \\ 
 \hline
\end{tabular}
\caption{Results for the spatial description resolution (SDR) task. Accuracy counts the proportion of instructions where the agent guesses within $9.14$ pixels of the correct location in a scaled-down panorama of size $100{\times}464$.}
\vspace{-15pt}
\end{center}
\end{table}



\paragraph{Navigation Tasks} \dm{Explain the result} 

\begin{table}[]
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|}
    \hline
    \textbf{Method} & \multicolumn{3}{c|}{\textbf{Dev}} & \multicolumn{3}{c|}{\textbf{Train}} \\
    \hline
    & \textbf{SPD} & \textbf{ND} & \textbf{TC}& \textbf{SPD} & \textbf{ND} & \textbf{TC}\\
    \hline
        Stop &  28.6 & 26.7 & 0 & 28.8 & 26.9 & 0\\
        Random Walk & 28.6 & 26.8 & 0.2 & 28.8 & 26.9 & 0.2\\
        \hline 
        Deep Mind + Supervised & 25.1 & 23.4 & 6.8 & 11.9 & 10.9 & 37.7\\
        Deep Mind + Supervised (Overfitting) & 26.3 & 24.6 & \textbf{8} & \textbf{1.2} & \textbf{1.1} & \textbf{94.2} \\
        Deep Mind + Mixture & \textbf{23.1} & \textbf{21.5} & 5.9 & 14.8 & 13.6 & 26.4 \\
        \hline
    \end{tabular}
    \caption{Dev and Train results on the navigation task.}
    \label{tab:my_label}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{|l|c|}
        \hline
        \textbf{Method} & \textbf{SPD} \\
        \hline
        Stop &  45.2\\
        Random Walk & 45.13\\
        Move Forward & 85.97\\
        \hline 
        Chaplot et al. + Contextual bandit & 45.23\\
        Chaplot et al. + Supervised & \\
        Chaplot et al. + A3C & \\
        Misra et al. & \\
        Deep Mind et al.  + Contextual Bandit & 45.22\\
        \hline
        Decouple Attention similar to EMNLP & \\
        \hline
    \end{tabular}
    \caption{Dev results on the navigation task.}
    \label{tab:my_label}
\end{table}


\begin{table}[]
    \centering
    \begin{tabular}{|l|c|}
    \hline
    \textbf{Method} & \textbf{SPD} \\
    \hline
        Stop &  45.75\\
        Random Walk & 45.69\\
        Move Forward & 86.76\\
        \hline 
        Chaplot et al. + Contextual Bandit & 45.75 \\
        Chaplot et al. + Supervised & \\
        Chaplot et al. + A3C & \\
        Misra et al. & \\
        Deep Mind et al.  + Contextual Bandit & 45.75\\
        \hline
         Decouple Attention similar to EMNLP & \\
        \hline
    \end{tabular}
    \caption{Test results on the navigation task.}
    \label{tab:my_label}
\end{table}



==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}
